VideoICL: Confidence-based Iterative In-context Learning for Out-of-Distribution Video Understanding

Recent advancements in video large multimodal models (LMMs) have significantly improved their video understanding and reasoning capabilities. However, their performance drops on out-of-distribution (OOD) tasks that are underrepresented in training data. Traditional methods like fine-tuning on OOD datasets are impractical due to high computational costs. While In-context learning (ICL) with demonstration examples has shown promising generalization performance in language tasks and image-language tasks without fine-tuning, applying ICL to video-language tasks faces challenges due to the limited context length in Video LMMs, as videos require longer token lengths. To address these issues, we propose VideoICL, a novel video in-context learning framework for OOD tasks that introduces a similarity-based relevant example selection strategy and a confidence-based iterative inference approach. This allows to select the most relevant examples and rank them based on similarity, to be used for inference. If the generated response has low confidence, our framework selects new examples and performs inference again, iteratively refining the results until a high-confidence response is obtained. This approach improves OOD video understanding performance by extending effective context length without incurring high costs. The experimental results on multiple benchmarks demonstrate significant performance gains, especially in domain-specific scenarios, laying the groundwork for broader video comprehension applications. Code will be released at https://github.com/KangsanKim07/VideoICL

==> tables/tab_ablation_nshots.tex <==
\begin{table}[t!]
    \setlength{\shiftdown}{-0.3em}
    \newcommand{\grey}[1]{\cellcolor[HTML]{eeeeee}{#1}}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccc}
        \toprule
         & \multirow{2}{*}[\shiftdown]{\makecell{Animal\\\small Kingdom}} & \multirow{2}{*}[\shiftdown]{\makecell{Pit-\\VQA}} & \multirow{2}{*}[\shiftdown]{\makecell{UCF-\\Crime}} & \multicolumn{3}{c}{CapERA} \\
         \cmidrule(l{2pt}r{2pt}){5-7}
         &&&& {\scriptsize BLEU-3} & {\scriptsize METEOR} & {\scriptsize ROUGE-L} \\
         \midrule
         \makecell[l]{Baseline} & 68.0 & 6.7 &  39.3 & 0.027 & 0.149 & 0.181 \\
         \midrule
         \textbf{$m=k/4$} & & & & & &  \\
         \grey{$\Delta$} & \grey{} & \grey{} & \grey{} & \grey{} & \grey{} & \grey{}  \\
         \textbf{$m=k/2$} & & & & & &  \\
         \grey{$\Delta$} & \grey{} & \grey{} & \grey{} & \grey{} & \grey{} & \grey{}  \\
         \textbf{$m=k$} & & & & & &  \\
         \grey{$\Delta$} & \grey{} & \grey{} & \grey{} & \grey{} & \grey{} & \grey{}  \\
         \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation on the number of demonstrations per iteration ($m$).}}
    \label{tab:ablation_nshots}
\end{table}

==> tables/tab_proprietary.tex <==
\begin{table*}[t!]
    \setlength{\shiftdown}{-0.3em}
    \newcommand{\grey}[1]{\cellcolor[HTML]{eeeeee}{#1}}
    \centering
    \resizebox{0.6\linewidth}{!}{
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{lcccccc}
        \toprule
         & \multirow{2}{*}[\shiftdown]{\makecell{Animal\\\small Kingdom}} & \multirow{2}{*}[\shiftdown]{\makecell{Pit-\\VQA}} & \multirow{2}{*}[\shiftdown]{\makecell{UCF-\\Crime}} & \multicolumn{2}{c}{CapERA} & \\
         \cmidrule(l{2pt}r{2pt}){5-6}
         &&&& {\scriptsize BLEU-4} & {\scriptsize METEOR} & \multirow{-2}{*}{Avg.} \\
         \midrule
         \makecell[l]{GPT-4o~\citep{openai_gpt-4o_2024}} & 
         58.2 & 6.9 & \textbf{58.0} & 0.023 & 0.142 & \grey{28.0} \\
         Gemini-1.5 Pro~\citep{geminiteam2024gemini15unlockingmultimodal}& 
         \textbf{72.9} & 14.7 & 55.1 & 0.019 & 0.134 & \grey{31.6} \\
         \textbf{\ours (Ours)} & 
         72.3 & \textbf{61.3} & 53.3 & \textbf{0.170} & \textbf{0.253} & \grey{\textbf{45.8}} \\
         \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Comparison with Proprietary APIs.} \ours uses the LLaVa-Video-7B~\citep{zhang_video_2024} model as the backbone. The highest scores for each benchmark are shown in bold.}
    \label{tab:proprietary}
\end{table*}
